Optical Flow Estimation in the Deep Learning Age

Akin to many subareas of computer vision, the recent advances in deep learning have also significantly influenced the literature on optical flow. Previously, the literature had been dominated by classical energy-based models, which formulate optical flow estimation as an energy minimization problem. However, as the practical benefits of Convolutional Neural Networks (CNNs) over conventional methods have become apparent in numerous areas of computer vision and beyond, they have also seen increased adoption in the context of motion estimation to the point where the current state of the art in terms of accuracy is set by CNN approaches. We first review this transition as well as the developments from early work to the current state of CNNs for optical flow estimation. Alongside, we discuss some of their technical details and compare them to recapitulate which technical contribution led to the most significant accuracy improvements. Then we provide an overview of the various optical flow approaches introduced in the deep learning age, including those based on alternative learning paradigms (e.g., unsupervised and semi-supervised methods) as well as the extension to the multi-frame case, which is able to yield further accuracy improvements.

==> preamble.tex <==
\usepackage[ngerman,main=english]{babel}

% Fix by https://tex.stackexchange.com/a/441701/9075
\usepackage{regexpatch}
\makeatletter
\edef\switcht@albion{%
  \relax\unexpanded\expandafter{\switcht@albion}%
}
\xpatchcmd*{\switcht@albion}{ \def}{\def}{}{}
\xpatchcmd{\switcht@albion}{\relax}{}{}{}
\edef\switcht@deutsch{%
  \relax\unexpanded\expandafter{\switcht@deutsch}%
}
\xpatchcmd*{\switcht@deutsch}{ \def}{\def}{}{}
\xpatchcmd{\switcht@deutsch}{\relax}{}{}{}
\edef\switcht@francais{%
  \relax\unexpanded\expandafter{\switcht@francais}%
}
\xpatchcmd*{\switcht@francais}{ \def}{\def}{}{}
\xpatchcmd{\switcht@francais}{\relax}{}{}{}
\makeatother

% better font, similar to the default springer font
% cfr-lm is preferred over lmodern. Reasoning at http://tex.stackexchange.com/a/247543/9075
% \usepackage[%
%   rm={oldstyle=false,proportional=true},%
%   sf={oldstyle=false,proportional=true},%
%   tt={oldstyle=false,proportional=true,variable=false},%
%   qt=false%
% ]{cfr-lm}
% \usepackage[T1]{fontenc}

\usepackage{graphicx}
\usepackage{booktabs}

%enable margin kerning
% \RequirePackage[babel,final,expansion=alltext,protrusion=alltext-nott]{microtype}
  
% Required for package pdfcomment later
\usepackage{xcolor}
\usepackage{pdfcomment}

% Doc: http://texdoc.net/natbib
\usepackage[
  square,        % for square brackets
  comma,         % use commas as separators
  numbers,       % for numerical citations;
%  sort,          % orders multiple citations into the sequence in which they appear in the list of references;
  sort&compress, % as sort but in addition multiple numerical citations are compressed if possible (as 3-6, 15);
]{natbib}
\renewcommand{\bibnumfmt}[1]{#1.}

% Prepare more space-saving rendering of the bibliography
% Source: https://tex.stackexchange.com/a/280936/9075
% \SetExpansion
% [ context = sloppy,
%   stretch = 30,
%   shrink = 60,
%   step = 5 ]
% { encoding = {OT1,T1,TS1} }
% { }

% Put footnotes below floats
\usepackage{stfloats}
\fnbelowfloat

%% ----------------------------------------------------------------------------------------------- %%
%% Our custom Package 
\usepackage{tikz}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{subcaption}
\captionsetup{compatibility=false}
\captionsetup{font=footnotesize}
\usepackage{amsmath,amssymb}
% \usepackage{newtxmath}       % selects Times Roman as basic font
\usepackage{tabularx}
\graphicspath{{../}}
%% ----------------------------------------------------------------------------------------------- %%

\usepackage{etoolbox,siunitx}
\robustify\bfseries
\sisetup{detect-all=true,group-four-digits,per-mode=fraction}


\usepackage{hyperref}
\hypersetup{hidelinks,colorlinks=true,pdfstartview=Fit,breaklinks=true}
% \hypersetup{hidelinks,colorlinks=true,allcolors=black,pdfstartview=Fit,breaklinks=true}

% Enable correct jumping to figures when referencing
\usepackage[all]{hypcap}
\usepackage[capitalise,nameinlink]{cleveref}

%Nice formats for \cref
\crefname{section}{Sect.}{Sect.}
\Crefname{section}{Section}{Sections}

%Intermediate solution for hyperlinked refs. See https://tex.stackexchange.com/q/132420/9075 for more information.
\newcommand{\Vlabel}[1]{\label[line]{#1}\hypertarget{#1}{}}
\newcommand{\lref}[1]{\hyperlink{#1}{\FancyVerbLineautorefname~\ref*{#1}}}

\usepackage{xspace}
\newcommand{\etal}{\textit{et al}.}
\newcommand{\ie}{\textit{i}.\textit{e}.}
\newcommand{\eg}{\textit{e}.\textit{g}.}

% Enable copy and paste - also of numbers,https://tex.stackexchange.com/a/430599/9075
\input glyphtounicode
\pdfgentounicode=1

